CrypQ: A Database Benchmark Based on Dynamic, Ever-Evolving Ethereum Data

Modern database systems are expected to handle dynamic data whose characteristics may evolve over time. Many popular database benchmarks are limited in their ability to evaluate this dynamic aspect of the database systems. Those that use synthetic data generators often fail to capture the complexity and unpredictable nature of real data, while most real-world datasets are static and difficult to create high-volume, realistic updates for. This paper introduces CrypQ, a database benchmark leveraging dynamic, public Ethereum blockchain data. CrypQ offers a high-volume, ever-evolving dataset reflecting the unpredictable nature of a real and active cryptocurrency market. We detail CrypQ's schema, procedures for creating data snapshots and update sequences, and a suite of relevant SQL queries. As an example, we demonstrate CrypQ's utility in evaluating cost-based query optimizers on complex, evolving data distributions with real-world skewness and dependencies.

==> old/app-schema.tex <==
\section{Detailed Schema Description}
\label{app:schema}

\begin{center}
\begin{tabular}{ |p{3cm}|p{9.5cm}|  }
 \hline
 \multicolumn{2}{|c|}{Withdrawals table} \\
 \hline
 hash & The hash (unique identifier) of the block in which this withdrawal occurred\\ \hline
 withdrawal\_index & The index of this withdrawal out of all withdrawals that occurred in this block\\ \hline
 validator & A user that has locked up at least 32 Ether to participate in staking. This is a special id given to the validator\\ \hline
 address & Address of the validator\\ \hline
 amount    & Amount withdrawn\\
 \hline
\end{tabular}
\end{center}

 \begin{center}
\begin{tabular}{ |p{3cm}|p{9.5cm}|  }
 \hline
 \multicolumn{2}{|c|}{Addresses table} \\
 \hline
address & Represents either a user or a contract \\ \hline
 eth\_balance & The ether balance of this address\\ \hline
\end{tabular}
\end{center}

 \begin{center}
\begin{tabular}{ |p{3cm}|p{9.5cm}|  }
 \hline
 \multicolumn{2}{|c|}{Blocks table} \\
 \hline
hash & Hash of the block, this is unique and allows it to be distinguished from other blocks \\ \hline
number & The sequential number of this block among all existing blocks \\ \hline
timestamp & The timestamp at which this block was added to the blockchain \\ \hline
extra\_data & Any extra data included in this block \\ \hline
base\_fee\_per\_gas & This is the base fee that all transactions in this block had to pay. Depending on the amount of transactions in the previous block, this number is adjusted up or down \\ \hline
size & The size of this block in bytes \\ \hline
miner & Also known as validator. This is the address of the user that successfully validated this block \\ \hline
\end{tabular}
\end{center}

 \begin{center}
\begin{tabular}{ |p{3cm}|p{9.5cm}|  }
 \hline
 \multicolumn{2}{|c|}{Transactions table} \\
 \hline
hash & Hash of the transaction, this is unique and allows a transaction to be distinguished from other transactions \\ \hline
 transaction\_index & The sequential number of this transaction among other transactions in the same block \\ \hline
value & The total value transferred in Wei in this transaction. $10^{18}$ Wei is one Ether \\ \hline
 from\_address & The address of the sender \\ \hline
to\_address & The address of a receiver \\ \hline
 gas & Units of gas required for this transaction \\ \hline
max\_priority\_fee\_ per\_ gas & On top of the base\_fee\_per\_gas which is the same for all transactions in a block, a sender may wish to pay extra to incentivize validators to include their transaction in the given block. This is represented by the priority fee. \\ \hline
 input & Data sent along with the transaction \\ \hline
block\_hash & The hash of the block in which this transaction took place \\ \hline
 transaction\_type & There are 128 possible transaction types, numbered between 0 and 0x7f: https://ethereum.org/en/developers/docs/transactions/ \\ \hline
nonce & Nonce is used to prevent double spending. This is the number of transactions sent from the sender’s address up to this point \\ \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ |p{3cm}|p{9.5cm}|  }
 \hline
 \multicolumn{2}{|c|}{Contracts table} \\
 \hline
address & Address of the contract \\ \hline
version & It is possible to exploit certain mechanisms and deploy different contracts at the same address. In order to deal with this loophole, version along with address helps to uniquely identify a given contract \\ \hline
function\_ signhashes & 4 byte hash of the function signature \\ \hline
bytecode & Bytecode of the contract \\ \hline
is\_erc20 & Boolean value to indicate if this is a contract of type ERC20 \\ \hline
is\_erc721 & Boolean value to indicate if this is a contract of type ERC721 \\ \hline
block\_hash & The hash of the block in which this contract was created \\ \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ |p{3cm}|p{9.5cm}|  }
 \hline
 \multicolumn{2}{|c|}{Tokens table} \\
 \hline
address & Address of the token \\ \hline
symbol & Symbol of the token \\ \hline
name & Name of the token \\ \hline
decimals & The number of decimal places the token uses \\ \hline
total\_supply & Total supply of the token \\ \hline
block\_hash & Hash of the block in which this token was created \\ \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ |p{3cm}|p{9.5cm}|  }
 \hline
 \multicolumn{2}{|c|}{Token Transactions table} \\
 \hline
transaction\_hash & Hash of the transaction in which this event occurred \\ \hline
log\_index & Index of this particular token transaction in the logs of the block in which this transaction occurred. Within one transaction, there can exist multiple different token transactions which is why this also has to be included in the primary key \\ \hline
token\_address & Address of the token that was transacted \\ \hline
value & The quantity of the token transferred \\ \hline
\end{tabular}
\end{center}

